HoGS: Unified Near and Far Object Reconstruction via Homogeneous Gaussian Splatting

Novel view synthesis has demonstrated impressive progress recently, with 3D Gaussian splatting (3DGS) offering efficient training time and photorealistic real-time rendering. However, reliance on Cartesian coordinates limits 3DGS's performance on distant objects, which is important for reconstructing unbounded outdoor environments. We found that, despite its ultimate simplicity, using homogeneous coordinates, a concept on the projective geometry, for the 3DGS pipeline remarkably improves the rendering accuracies of distant objects. We therefore propose Homogeneous Gaussian Splatting (HoGS) incorporating homogeneous coordinates into the 3DGS framework, providing a unified representation for enhancing near and distant objects. HoGS effectively manages both expansive spatial positions and scales particularly in outdoor unbounded environments by adopting projective geometry principles. Experiments show that HoGS significantly enhances accuracy in reconstructing distant objects while maintaining high-quality rendering of nearby objects, along with fast training speed and real-time rendering capability. Our implementations are available on our project page https://kh129.github.io/hogs/.

==> figures/psnr_curve.tex <==
\begin{figure*}
  \centering
  \resizebox{1.00\linewidth}{!}{
  \begin{tabular}{cc}
    \includegraphics[width=0.325\textwidth]{figures/src/psnr_plot_train.pdf} &
    \includegraphics[width=0.325\textwidth]{figures/src/psnr_plot_test.pdf} \\
    \multicolumn{1}{c}{(a) PSNR curve on train dataset} & \multicolumn{1}{c}{(b) PSNR curve on test dataset}
  \end{tabular}
}\vspace{-2mm}
\caption{
\textbf{PSNR curve on train and test dataset.} }\vspace{-2mm}
\label{fig:sim1d}
\end{figure*}

==> figures/qualitative_analysis.tex <==
\clearpage % Start a new page
\begin{figure*}[t]
  \centering
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
    \includegraphics[width=\textwidth]{figures/src/tentative/qualitative_analysis.pdf}\vspace{-2mm}
    \captionsetup{width=\textwidth} % Set caption width to text width
   \caption{
   \textbf{Visual Comparisons on Novel View Synthesis.} We show comparisons of our method with previous methods on test views.  The figure includes KITCHEN and TREEHILL from the Mip-NeRF360 dataset; TRAIN and TRUCK from Tanks\&Temples; and scene 21, 26, 69 and 97 from DL3DV benchmark. The first two sets of views are bounded indoor scenes, and the rest are unbounded outdoor scenes.
   }\vspace{-2mm}
   \label{fig:qualitative}
\end{figure*}
\clearpage % Start a new page

==> tables/ablation_12.tex <==
\begin{table*}[t!]
  \small
\resizebox{1.0\linewidth}{!}{
  \tabcolsep=0.07cm
  \begin{tabular}{c|ccc|ccc|ccc}\hline
    Dataset & \multicolumn{3}{c|}{Train}  & \multicolumn{3}{c|}{Scene 21 DL3DV} & \multicolumn{3}{c}{Scene 97 DL3DV}\\
    Ablation \textbar{} Metric
    & $SSIM^\uparrow$   & $PSNR^\uparrow$    & $LPIPS^\downarrow$
    & $SSIM^\uparrow$   & $PSNR^\uparrow$    & $LPIPS^\downarrow$ 
    & $SSIM^\uparrow$   & $PSNR^\uparrow$    & $LPIPS^\downarrow$ \\
\hline
    w/o Homog. Scaling& 0.825 & 22.44 &  0.194 & 0.872 & 27.79 & 0.148 & 0.953 & 33.09 & 0.092  \\
    w/ Pruning& 0.823           & 22.31 &          0.196 &        0.868 &        27.34 &       0.156 &        0.950 &         31.97 &        0.096 \\ 
 \hline
    Ours & 0.828 & 22.60 & 0.191  & 0.872 & 27.80 & 0.148 & 0.953 & 33.12 & 0.092  \\
    \hline
  \end{tabular}
  }\vspace{-2mm}
  \caption{
    \textbf{Comparative Analysis of Novel View Synthesis Techniques.} Placeholder caption: Ablation Table Overall Metrics.
  }\vspace{-2mm}
  \label{tab:ablation_normal}
\end{table*}


==> tables/ablation_12_far.tex <==
\begin{table*}[t!]
  \small
\resizebox{1.0\linewidth}{!}{
  \tabcolsep=0.07cm
  \begin{tabular}{c|ccc|ccc|ccc}\hline
    Dataset & \multicolumn{3}{c|}{Train}  & \multicolumn{3}{c|}{Scene 21 DL3DV} & \multicolumn{3}{c}{Scene 97 DL3DV}\\
    Ablation \textbar{} Metric
    & $SSIM^\uparrow$   & $PSNR^\uparrow$    & $LPIPS^\downarrow$
    & $SSIM^\uparrow$   & $PSNR^\uparrow$    & $LPIPS^\downarrow$ 
    & $SSIM^\uparrow$   & $PSNR^\uparrow$    & $LPIPS^\downarrow$ \\
\hline
    w/o Homog. Scaling& 0.973 & 30.23 &  0.047 & \textbf{0.986} & 35.46 & \textbf{0.022} & \textbf{0.992} & 40.11 & \textbf{0.039}  \\
    w/ Pruning& 0.971           & 29.51 &          0.050 &        0.983 &        33.76 &       0.028 &        0.990 &         37.28 &        0.043 \\ 
 \hline
    Ours & \textbf{0.976} & \textbf{30.43} & \textbf{0.044}  & \textbf{0.986} & \textbf{35.48} & \textbf{0.022} & \textbf{0.992} & \textbf{40.41} & \textbf{0.039}  \\
    \hline
  \end{tabular}
  }\vspace{-2mm}
  \caption{
    \textbf{Comparative Analysis of Novel View Synthesis Techniques using Far Metrics.} 
    Placeholder caption: Ablation Table Far Metrics.
  }\vspace{-2mm}
  \label{tab:ablation}
\end{table*}


==> tables/ablation_12_psnr.tex <==
% \begin{table*}[t!]
%   \small
% \resizebox{1.0\linewidth}{!}{
%   \tabcolsep=0.07cm
%   \begin{tabular}{c|c|c|c}\hline
%     Dataset & Train  & Scene 21 DL3DV & Scene 97 DL3DV\\
%     Ablation \textbar{} Metric
%     & $PSNR^\uparrow$    
%     & $PSNR^\uparrow$    
%     & $PSNR^\uparrow$    \\
% \hline
%     w/o Homog. Scaling& 30.23 & 35.46 & 40.11  \\
%     w/ Pruning& 29.51 & 33.76 & 37.28 \\ 
%  \hline
%     Ours & \textbf{30.43} & \textbf{35.48} & \textbf{40.41}  \\
%     \hline
%   \end{tabular}
%   }
%   \caption{
%     \textbf{Comparative Analysis of Novel View Synthesis Techniques using PSNR Metric.} 
%     Placeholder caption: Ablation Table PSNR Metric.
%   }
%   \label{tab:ablation}
% \end{table*}


\begin{table}[t!]
  \small
\resizebox{\linewidth}{!}{
  \tabcolsep=0.07cm
  \begin{tabular}{c|c|c|c}\hline
     & Train  & DL3DV-21 & DL3DV-97 \\
\hline
    w/o Homog. Scaling & 30.23 & 35.46 & 40.11  \\
    w/ Pruning & 29.51 & 33.76 & 37.28 \\ 
 \hline
    Ours & \textbf{30.43} & \textbf{35.48} & \textbf{40.41}  \\
    \hline
  \end{tabular}
  }\vspace{-2mm}
  \caption{
    \textbf{Comparative Analysis of Novel View Synthesis Techniques using far PSNR Metric.} 
    Placeholder caption: Ablation Table PSNR Metric.
  }\vspace{-2mm}
  \label{tab:ablation}
\end{table}


==> tables/quantitative_in_and_out.tex <==
% \begin{table}[t!]
% \centering
% \small
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{>{\centering\arraybackslash}m{3cm}|c|ccc|ccc}
% \hline
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Metrics} & \multicolumn{3}{c|}{Indoor Scene} & \multicolumn{3}{c}{Outdoor Scene} \\ 
% \cline{3-8} 
%  & & Zip-NeRF & 3DGS & Ours & Zip-NeRF & 3DGS & Ours \\ 
% \hline
% \multirow{3}{*}{\makecell{Mip-NeRF360\\ Dataset}} 
%     & $SSIM^\uparrow$    & \wll{0.929} & \wll{0.929} & \wll{0.930} & \wll{0.748} & \wll{0.734} & \wll{0.747} \\
%     & $PSNR^\uparrow$    & \wll{32.33} & \wll{31.24} & \wll{31.38} & \wll{25.54} & \wll{24.78} & \wll{25.14} \\
%     & $LPIPS^\downarrow$ & \wll{0.161} & \wll{0.169} & \wll{0.163} & \wll{0.209} & \wll{0.246} & \wll{0.219} \\ 
% \hline
% \end{tabular}
% }
% \caption{Quantitative results on Mip-NeRF 360~\cite{mipnerf360} dataset. \textbf{White cells} indicate metrics for `indoor` regions, while \textbf{gray cells} indicate metrics for `outdoor` regions.}
% \label{tab:in_out}
% \end{table}

\begin{table}[t!]
\centering
\small
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{Indoor} & \multicolumn{3}{c}{Outdoor} \\ 
\cline{2-7} 
 & SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ & SSIM$^\uparrow$ & PSNR$^\uparrow$ & LPIPS$^\downarrow$ \\ 
\hline
Zip-NeRF    & \wll{0.929} & \wll{32.33} & \wll{0.161} & \wll{0.748} & \wll{25.54} & \wll{0.209} \\
3DGS        & \wll{0.929} & \wll{31.24} & \wll{0.169} & \wll{0.734} & \wll{24.78} & \wll{0.246} \\
Scaffold-GS & \wll{0.933} & \wll{31.59} & \wll{0.161} & \wll{0.744} & \wll{24.78} & \wll{0.225} \\
\HGS (Ours) & \wll{0.930} & \wll{31.38} & \wll{0.163} & \wll{0.747} & \wll{25.14} & \wll{0.219} \\
\hline
\end{tabular}
}\vspace{-2mm}
\caption{Quantitative results on Mip-NeRF 360~\cite{mipnerf360} indoor and outdoor scenes, showing the strong results by \HGS for general outdoor scenes.}\vspace{-2mm}
\label{tab:in_out}
\end{table}


% dont delete this table!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

% \begin{table}[t!]
% \centering
% \small
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{>{\centering\arraybackslash}m{3cm}|c|cc|cc}
% \hline
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Metrics} & \multicolumn{2}{c|}{Indoor Scene} & \multicolumn{2}{c}{Outdoor Scene} \\ 
% \cline{3-6} 
%  & & 3DGS & Ours & 3DGS & Ours \\ 
% \hline
% \multirow{3}{*}{\makecell{Mip-NeRF360\\ Dataset}} 
%     & $SSIM^\uparrow$    & \wll{0.929} & \wll{0.930} &  \wll{0.734} & \wll{0.747} \\
%     & $PSNR^\uparrow$    & \wll{31.24} & \wll{31.38} &  \wll{24.78} & \wll{25.14} \\
%     & $LPIPS^\downarrow$ & \wll{0.169} & \wll{0.163} &  \wll{0.246} & \wll{0.219} \\ 
% \hline
% \end{tabular}
% }
% \caption{Comparison of metrics between models. \textbf{White cells} indicate metrics for `indoor` regions, while \textbf{gray cells} indicate metrics for `outdoor` regions.}
% \label{tab:in_out}
% \end{table}
